Each Attribute Matters: Contrastive Attention for Sentence-based Image Editing

Sentence-based Image Editing (SIE) aims to deploy natural language to edit an image. Offering potentials to reduce expensive manual editing, SIE has attracted much interest recently. However, existing methods can hardly produce accurate editing and even lead to failures in attribute editing when the query sentence is with multiple editable attributes. To cope with this problem, by focusing on enhancing the difference between attributes, this paper proposes a novel model called Contrastive Attention Generative Adversarial Network (CA-GAN), which is inspired from contrastive training. Specifically, we first design a novel contrastive attention module to enlarge the editing difference between random combinations of attributes which are formed during training. We then construct an attribute discriminator to ensure effective editing on each attribute. A series of experiments show that our method can generate very encouraging results in sentence-based image editing with multiple attributes on CUB and COCO dataset. Our code is available at https://github.com/Zlq2021/CA-GAN

==> p5.tex <==
\section{Related Work}

% \subsection{Text-to-image generation }
% The purpose of Text-to-Image Generation is to generate the corresponding image from text description. 
% Nguyen \etal\cite{nguyen2017plug} introduced a sampling method similar to Langevin to synthesize images from text. 
% Xu \etal\cite{xu2018attngan} proposed multi-stage AttnGANs, which synthesize different parts of a scene by focusing on different words in a text. In the first stage, the generator uses sentence embedding to synthesize images. 
% In the next stage, the contextual features of words are calculated by the attention model and input to the next generator. 
% Qiao \etal\cite{qiao2019mirrorgan} introduced a mirror to connect the dual tasks of text-image synthesis and text subtitles and constrained the reproduced subtitles to align with the given subtitles. In the task of generating images with various features, Zhang \etal\cite{zhang2017stackgan,zhang2018stackgan++} transformed the complex generation problem into several sub-problems, and gradually synthesized and refined images by using multiple generators arranged in a tree structure. 
% However, all the above methods mainly focus on generating new images from text, rather than using natural language description to manipulate specific visual attributes of a given image. 
% And when the image contains multiple features, multiple generators are needed. 
% By comparing the construction of loss, we train a generator, which can manipulate multiple feature information simultaneously according to text information.

\subsection{Sentence-based image editing}
In recent years, based on Generative Adversarial Networks (GANs)~\cite{zhu2019dm,zhang2018photographic,yin2019semantics,tan2019semantics,qiao2019learn,lao2019dual}, scientists pay more attention to the image generation or transformation from text or other images, such as Text-to-Image Generation~\cite{nguyen2017plug,xu2018attngan,qiao2019mirrorgan,zhang2017stackgan,zhang2018stackgan++} and Image-to-Image Translation~\cite{ye2019unsupervised}.
To make the transformation controllable, Text-based Image Editing will only edit the target area of the image through text description. 
Generally, the query text can be a word, a short phrase or a long sentence.
Dong \etal\cite{dong2017semantic} proposed an encoder-decoder structure to edit images matched with a given text. 
In order to keep the content irrelevant to the text in the original image, \cite{vo2018paired} proposed to construct foreground and background distribution with different recognizers. 
Nam \etal\cite{nam2018text} eliminated different visual attributes by introducing a text adaptive discriminator, which can provide more detailed training feedback to the generator. 
Li \etal\cite{li2020manigan} adopt the structure of the multi-level network, and can generate high-quality image content through the combination module of ACM and DCM. 
However, the generators of these methods ignore the difference between long sentences with word and phrase that the sentences may contain multiple editable attributes.
In this paper, we focus on the Sentence-based Image Editing (SIE), and propose to construct Contrastive Attention to enhance the attribute editing.

\subsection{Contrastive learning}
% Contrastive learning is widely used in self-supervised representational learning~. 
For a given anchor point in the data, the purpose of contrast learning~\cite{yu2019multi,he2020momentum,chen2020simple} is to bring the anchor point closer to the positive point and push the anchor point farther away to the negative point in the representation space, thus enhancing the consistency of the feature representation. 
In previous vision tasks~\cite{wu2018unsupervised,lee2021infomax,deng2020disentangled,kang2020contragan}, the idea of contrast learning is also used because of the relationship between positive and negative samples of data samples. 
It was also demonstrated in~\cite{park2020contrastive} that contrast learning methods are effective in the task of image to image conversion. 
Some works also studied the contrastive training in nature language processing~\cite{?}.
In contrast to the above work, we apply the idea of contrast learning to the task of text-editing images by the proposed Contrastive Attention.
The Contrastive Attention is based on the fact that different attribute edits different.



